Iris in Lean

The Iris framework for concurrent separation logic has been widely used for program verification research. An important factor contributing to the framework's adoption is its high-quality mechanization in Rocq. This mechanization uses a number of Rocq features in sophisticated ways, including a carefully constructed algebraic hierarchy for modeling separation logic resources, and a proof mode for embedded separation logic proofs, which combines custom Ltac with extensible typeclasses. The library has been developed for over a decade with dozens of contributors, with an emphasis on modularity and maintainability. We explore how Lean features like flexible metaprogramming and quotient types can simplify the design and usage of Iris. Using these features, we provide a novel implementation of the Iris proof mode with improved performance, simplify the handling of equivalences through quotient types, build a variant of Diaframe proof automation, and provide convenience features like automatic construction of Iris fixed points. Building on Lean lets us integrate with the extensive Mathlib library, allowing us to re-use results from this library for program verification tasks that have heavy mathematical dependencies, as we demonstrate with an application to probabilistic program verification.

==> lstlean.tex <==
% Listing style definition for the Lean Theorem Prover.
% Defined by Jeremy Avigad, 2015, by modifying Assia Mahboubi's SSR style.
% Unicode replacements taken from Olivier Verdier's unixode.sty

\lstdefinelanguage{lean} {

% Anything between $ becomes LaTeX math mode
mathescape=false,
% Comments may or not include Latex commands
texcl=false,

% keywords, list taken from lean-syntax.el
morekeywords=[1]{
import, prelude, protected, private, noncomputable, definition, meta, renaming,
hiding, parameter, parameters, begin, constant, constants,
lemma, variable, variables, theory,
print, theorem, example,
open, as, export, override, axiom, axioms, inductive, with,
structure, record, universe, universes,
alias, help, precedence, reserve, declare_trace, add_key_equivalence,
match, infix, infixl, infixr, notation, postfix, prefix, instance,
eval, reduce, check, end, this,
using, using_well_founded, namespace, section,
attribute, local, set_option, extends, include, omit, class,
raw, replacing,
calc, have, show, suffices, by, in, at, let, forall, Pi, fun,
exists, if, dif, then, else, assume, obtain, from, register_simp_ext, unless, break, continue,
mutual, do, def, run_cmd, const,
partial, mut, where, macro, syntax, deriving,
return, try, catch, for, macro_rules, declare_syntax_cat, abbrev,
rec,
ipm_class, ipm_tactic_instance, ipm_backtrack, rocq_alias,
elab, outParam, semiOutParamIPM, priority, low, high, tactic, step,

% tactics, moved from morekeywords=[3]
assumption,
apply, intro, intros, allGoals,
generalize, clear, revert, done, exact, specialize,
refine, repeat, cases, rewrite, rw, rcases,
simp, simp_all, dsimp, only, contradiction,
constructor, injection,
induction, unfold,
grind, rename,

% Iris
ifix, icofix, iguarded, iinductive,
wander, finish, sideconditions,
istart, istop,
irename, iclear, irevert, irevert!, ipure, iintuitionistic, ispatial,
iintro, icases, ihave, iexists, ileft, iright,
isplit, isplitl, isplitr, iframe, icombine,
iapply, ispecialize, iexact, iassumption, iaccu,
imodintro, inext, imod,
irewrite, ieval, isimp, iunfold, iloeb, iinduction, generalizing, generalizing!,
ipureintro, iempintro, iexfalso, itrivial,
iinv, iauintro, iaaccintro,

% Iris WP
wp_value_head, wp_expr_simp, wp_finish,
wp_bind,
wp_pure, wp_pures,
wp_rec,
wp_if, wp_if_true, wp_if_false,
wp_unop, wp_binop, wp_op,
wp_lam, wp_let, wp_seq,
wp_proj, wp_case, wp_inj, wp_pair,
wp_closure, wp_match,
wp_apply_raw, wp_smart_apply_raw, wp_apply_post, wp_apply, wp_smart_apply,
wp_load, wp_store, wp_alloc, wp_free,
wp_xchg, wp_faa, wp_cmpxchg_suc, wp_cmpxchg_fail, wp_cmpxchg,
},

alsoletter={!}

% Sorts
morekeywords=[2]{Sort, Type, Prop},

% Moved to [1] for consistency
morekeywords=[3]{},

% modifiers, taken from lean-syntax.el
% note: 'otherkeywords' is needed because these use a different symbol.
% this command doesn't allow us to specify a number -- they are put with [1]
% otherkeywords={
% [persistent], [notation], [visible], [instance], [trans_instance],
% [class], [parsing-only], [coercion], [unfold_full], [constructor],
% [reducible], [irreducible], [semireducible], [quasireducible], [wf],
% [whnf], [multiple_instances], [none], [decl], [declaration],
% [relation], [symm], [subst], [refl], [trans], [simp], [congr], [unify],
% [backward], [forward], [no_pattern], [begin_end], [tactic], [abbreviation],
% [reducible], [unfold], [alias], [eqv], [intro], [intro!], [elim], [grinder],
% [localrefinfo], [recursor]
% },

% Various symbols
literate=
% '^' stands for a literal '%' in listings, latexpand strips everything after a real '%'
{^}{{\%}}1
{α}{{\ensuremath{\mathrm{\alpha}}}}1
{β}{{\ensuremath{\mathrm{\beta}}}}1
{γ}{{\ensuremath{\mathrm{\gamma}}}}1
{δ}{{\ensuremath{\mathrm{\delta}}}}1
{ε}{{\ensuremath{\mathrm{\varepsilon}}}}1
{ζ}{{\ensuremath{\mathrm{\zeta}}}}1
{η}{{\ensuremath{\mathrm{\eta}}}}1
{θ}{{\ensuremath{\mathrm{\theta}}}}1
{ι}{{\ensuremath{\mathrm{\iota}}}}1
{κ}{{\ensuremath{\mathrm{\kappa}}}}1
{μ}{{\ensuremath{\mathrm{\mu}}}}1
{ν}{{\ensuremath{\mathrm{\nu}}}}1
{ξ}{{\ensuremath{\mathrm{\xi}}}}1
{π}{{\ensuremath{\mathrm{\mathnormal{\pi}}}}}1
{ρ}{{\ensuremath{\mathrm{\rho}}}}1
{σ}{{\ensuremath{\mathrm{\sigma}}}}1
{τ}{{\ensuremath{\mathrm{\tau}}}}1
{φ}{{\ensuremath{\mathrm{\varphi}}}}1
{χ}{{\ensuremath{\mathrm{\chi}}}}1
{ψ}{{\ensuremath{\mathrm{\psi}}}}1
{ω}{{\ensuremath{\mathrm{\omega}}}}1

{Γ}{{\ensuremath{\mathrm{\Gamma}}}}1
{Δ}{{\ensuremath{\mathrm{\Delta}}}}1
{Θ}{{\ensuremath{\mathrm{\Theta}}}}1
{Λ}{{\ensuremath{\mathrm{\Lambda}}}}1
{Σ}{{\ensuremath{\mathrm{\Sigma}}}}1
{Φ}{{\ensuremath{\mathrm{\Phi}}}}1
{Ξ}{{\ensuremath{\mathrm{\Xi}}}}1
{Ψ}{{\ensuremath{\mathrm{\Psi}}}}1
{Ω}{{\ensuremath{\mathrm{\Omega}}}}1

{ℵ}{{\ensuremath{\aleph}}}1

{≤}{{\ensuremath{\leq}}}1
{≥}{{\ensuremath{\geq}}}1
{≠}{{\ensuremath{\neq}}}1
{≈}{{\ensuremath{\approx}}}1
{≡}{{\ensuremath{\equiv}}}1
{≃}{{\ensuremath{\simeq}}}1

{«}{{\guillemotleft}}1
{»}{{\guillemotright}}1

{≤}{{\ensuremath{\leq}}}1
{≥}{{\ensuremath{\geq}}}1

{∂}{{\ensuremath{\partial}}}1
{∆}{{\ensuremath{\triangle}}}1 % or \laplace?

{∫}{{\ensuremath{\int}}}1
{∑}{{\ensuremath{\mathrm{\Sigma}}}}1
{Π}{{\ensuremath{\mathrm{\Pi}}}}1

{⊥}{{\ensuremath{\perp}}}1
{∞}{{\ensuremath{\infty}}}1
{∂}{{\ensuremath{\partial}}}1

{∓}{{\ensuremath{\mp}}}1
{±}{{\ensuremath{\pm}}}1
{×}{{\ensuremath{\times}}}1

{⊕}{{\ensuremath{\oplus}}}1
{⊗}{{\ensuremath{\otimes}}}1
{⊞}{{\ensuremath{\boxplus}}}1

{∇}{{\ensuremath{\nabla}}}1
{√}{{\ensuremath{\sqrt}}}1

{⬝}{{\ensuremath{\cdot}}}1
{•}{{\ensuremath{\cdot}}}1
{∘}{{\ensuremath{\circ}}}1

%{⁻}{{\ensuremath{^{\textup{\kern1pt\rule{2pt}{0.3pt}\kern-1pt}}}}}1
{⁻}{{\ensuremath{^{-}}}}1
{▸}{{\ensuremath{\blacktriangleright}}}1

{∧}{{\ensuremath{\wedge}}}1
{∨}{{\ensuremath{\vee}}}1
{¬}{{\ensuremath{\neg}}}1
{⊢}{{\ensuremath{\vdash}}}1
{⊣}{{\ensuremath{\dashv}}}1
{∗}{{\ensuremath{\ast}}}1
{⌜}{{\ensuremath{\ulcorner}}}1
{⌝}{{\ensuremath{\urcorner}}}1
{□}{{\ensuremath{\Box}}}1
{✓}{{\ensuremath{\checkmark}}}1

%{⟨}{{\ensuremath{\left\langle}}}1
%{⟩}{{\ensuremath{\right\rangle}}}1
{⟨}{{\ensuremath{\langle}}}1
{⟩}{{\ensuremath{\rangle}}}1

{↦}{{\ensuremath{\mapsto}}}1
{←}{{\ensuremath{\leftarrow}}}1
{<-}{{\ensuremath{\leftarrow}}}1
{→}{{\ensuremath{\rightarrow}}}1
{↔}{{\ensuremath{\leftrightarrow}}}1
{⇒}{{\ensuremath{\Rightarrow}}}1
{⟹}{{\ensuremath{\Longrightarrow}}}1
{⇐}{{\ensuremath{\Leftarrow}}}1
{⟸}{{\ensuremath{\Longleftarrow}}}1

{∩}{{\ensuremath{\cap}}}1
{∪}{{\ensuremath{\cup}}}1
{⊂}{{\ensuremath{\subseteq}}}1
{⊆}{{\ensuremath{\subseteq}}}1
{⊄}{{\ensuremath{\nsubseteq}}}1
{⊈}{{\ensuremath{\nsubseteq}}}1
{⊃}{{\ensuremath{\supseteq}}}1
{⊇}{{\ensuremath{\supseteq}}}1
{⊅}{{\ensuremath{\nsupseteq}}}1
{⊉}{{\ensuremath{\nsupseteq}}}1
{∈}{{\ensuremath{\in}}}1
{∉}{{\ensuremath{\notin}}}1
{∋}{{\ensuremath{\ni}}}1
{∌}{{\ensuremath{\notni}}}1
{∅}{{\ensuremath{\emptyset}}}1

{∖}{{\ensuremath{\setminus}}}1
{†}{{\ensuremath{\dag}}}1

{ℕ}{{\ensuremath{\mathbb{N}}}}1
{ℤ}{{\ensuremath{\mathbb{Z}}}}1
{ℝ}{{\ensuremath{\mathbb{R}}}}1
{ℚ}{{\ensuremath{\mathbb{Q}}}}1
{ℂ}{{\ensuremath{\mathbb{C}}}}1
{⌞}{{\ensuremath{\llcorner}}}1
{⌟}{{\ensuremath{\lrcorner}}}1
{⦃}{{\ensuremath{\{\!|}}}1
{⦄}{{\ensuremath{|\!\}}}}1

{‖}{{\ensuremath{\|}}}1
{₁}{{\ensuremath{_1}}}1
{₂}{{\ensuremath{_2}}}1
{₃}{{\ensuremath{_3}}}1
{₄}{{\ensuremath{_4}}}1
{₅}{{\ensuremath{_5}}}1
{₆}{{\ensuremath{_6}}}1
{₇}{{\ensuremath{_7}}}1
{₈}{{\ensuremath{_8}}}1
{₉}{{\ensuremath{_9}}}1
{₀}{{\ensuremath{_0}}}1
{ᵢ}{{\ensuremath{_i}}}1
{ⱼ}{{\ensuremath{_j}}}1
{ₐ}{{\ensuremath{_a}}}1

{¹}{{\ensuremath{^1}}}1

{ₙ}{{\ensuremath{_n}}}1
{ₘ}{{\ensuremath{_m}}}1
{ₚ}{{\ensuremath{_p}}}1
{↑}{{\ensuremath{\uparrow}}}1
{↓}{{\ensuremath{\downarrow}}}1

{...}{{\ensuremath{\ldots}}}1
{·}{{\ensuremath{\cdot}}}1

{Σ}{{\color{symbolcolor}\ensuremath{\Sigma}}}1
{Π}{{\color{symbolcolor}\ensuremath{\Pi}}}1
{∀}{{\color{symbolcolor}\ensuremath{\forall}}}1
{∃}{{\color{symbolcolor}\ensuremath{\exists}}}1
{λ}{{\color{symbolcolor}\ensuremath{\mathrm{\lambda}}}}1
{\$\$}{{\color{symbolcolor}\$\$}}2
{\$}{{\color{symbolcolor}\$}}1

{:=}{{\color{symbolcolor}:=}}1
{=}{{\color{symbolcolor}=}}1
{<|>}{{\color{symbolcolor}<|>}}1
{<\$>}{{\color{symbolcolor}<\$>}}1
{+}{{\color{symbolcolor}+}}1
{*}{{\color{symbolcolor}*}}1,

% Comments
%comment=[s][\itshape \color{commentcolor}]{/-}{-/},
morecomment=[s][\color{commentcolor}]{/-}{-/},
morecomment=[l][\itshape \color{commentcolor}]{--},

% Spaces are not displayed as a special character
showstringspaces=false,

% keep spaces
keepspaces=true,

% String delimiters
morestring=[b]",
morestring=[d],

% Size of tabulations
tabsize=3,

% Enables ASCII chars 128 to 255
extendedchars=false,

% Case sensitivity
sensitive=true,

% Automatic breaking of long lines
breaklines=true,
breakatwhitespace=true,

% Default style fors listingsred
basicstyle=\ttfamily\small,

% Position of captions is bottom
captionpos=b,

% Full flexible columns
columns=[l]fullflexible,


% Style for (listings') identifiers
identifierstyle={\ttfamily\color{black}},
% Note : highlighting of Coq identifiers is done through a new
% delimiter definition through an lstset at the beginning of the
% document. Don't know how to do better.

% Style for declaration keywords
keywordstyle=[1]{\ttfamily\color{keywordcolor}},

% Style for sorts
keywordstyle=[2]{\ttfamily\color{sortcolor}},

% Style for tactics keywords
keywordstyle=[3]{\ttfamily\color{tacticcolor}},

% Style for attributes
keywordstyle=[4]{\ttfamily\color{attributecolor}},

% Style for strings
stringstyle=\ttfamily,

% Style for comments
commentstyle={\ttfamily\footnotesize},

}


==> lstrocq.tex <==
%=======================================================================
% Définit le style ssr Gallina pour les listings (Assia Mahboubi 2007)

\lstdefinelanguage{coq} {
% Comments may or not include Latex commands
texcl=false,
frame=single,
keepspaces,
% Vernacular commands
morekeywords=[1]{
Polymorphic, Section, Module, End, Require, Import, Export,
Variable, Variables, Parameter, Parameters, Axiom, Hypothesis, Hypotheses,
Notation, Local, Tactic, Reserved, Scope, Open, Close, Bind, Delimit,
Definition, Let, Ltac, Fixpoint, CoFixpoint, Add, Morphism, Relation,
Implicit, Arguments, Contextual, Strict, Prenex, Implicits,
Iris, Inductive, CoInductive, Record, Structure, Canonical, Coercion,
Context, Class, Global, Instance, Program, Infix,
Theorem, Lemma, Corollary, Proposition, Fact, Remark, Example,
Proof, Goal, Save, Qed, Defined, Hint, Mode, Extern, Resolve, Rewrite, View,
Search, Show, Print, Printing, All, Graph, Projections, inside, outside, Eval,
Check},

% Gallina
morekeywords=[2]{match, with, end, if, then, else, let, in, as},
%morekeywords=[2]{forall, exists, exists2, fun, fix, cofix,
%      match, with, end, as, in, return, let, is, if, then, else,
%      for, of, nosimpl},

% Sorts
morekeywords=[3]{Set, Type, Prop, SProp},

% Various tactics, some are std Coq subsumed by ssr, for the manual purpose
morekeywords=[4]{
pose, set, move, case, elim, apply, clear,
hnf, intro, intros, generalize, rename, pattern, after,
destruct, induction, using, refine, inversion, injection,
rewrite, congr, unlock, compute, field, fourier,
replace, fold, unfold, change, cutrewrite, simpl,
have, suff, wlog, suffices, without, loss, nat_norm,
assert, cut, trivial, revert, bool_congr, nat_congr,
symmetry, transitivity, auto, split, left, right, autorewrite,
eauto, by, first, done, cbv, tc_solve,

% Iris
iStartProof, iStopProof,
iRename, iClear, iRevert, iPure, iIntuitionistic, iSpatial,
iIntros, iDestruct, iPoseProof, iExists, iLeft, iRight,
iSplit, iSplitL, iSplitR, iFrame, iCombine,
iApply, iSpecialize, iExact, iAssumption, iAccu,
iModIntro, iNext, iMod,
iRewrite, iEval, iSimp, iUnfold, iLöb, iInduction,
iPureIntro, iEmpIntro, iExFalso,
iInv, iAuIntro, iAaccIntro,

% Iris WP
wp_value_head, wp_expr_simp, wp_finish,
wp_bind,
wp_pure, wp_pures,
wp_rec,
wp_if, wp_if_true, wp_if_false,
wp_unop, wp_binop, wp_op,
wp_lam, wp_let, wp_seq,
wp_proj, wp_case, wp_inj, wp_pair,
wp_closure, wp_match,
wp_apply_raw, wp_smart_apply_raw, wp_apply_post, wp_apply, wp_smart_apply,
wp_load, wp_store, wp_alloc, wp_free,
wp_xchg, wp_faa, wp_cmpxchg_suc, wp_cmpxchg_fail, wp_cmpxchg,
},

% Terminators
%morekeywords=[5]{
%         by, done, exact, tauto, romega, omega,
%         assumption, solve, contradiction, discriminate},


% Control
%morekeywords=[6]{do, last, first, try, idtac, repeat},

morestring=[b]{"},

% Comments delimiters, we do turn this off for the manual
comment=[s]{(*}{*)},

% Spaces are not displayed as a special character
showstringspaces=false,

% Size of tabulations
tabsize=3,							

% Case sensitivity
sensitive=true,

% Automatic breaking of long lines
breaklines=true,

% Default style for listings
basicstyle=\small\ttfamily,

% Position of captions is bottom
captionpos=b,							

% Style for (listings') identifiers
identifierstyle={\ttfamily\color{purple!35!black}},
% Note : highlighting of Coq identifiers is done through a new
% delimiter definition through an lstset at the begining of the
% document. Don't know how to do better.

% Style for declaration keywords
keywordstyle=[1]{\ttfamily\color{blue!80!black}},
keywordstyle=[2]{\ttfamily},
keywordstyle=[3]{\ttfamily\color{red!80!black}},

%Style for iterators
%keywordstyle=[6]{\ttfamily\color{dkpink}},

% Style for strings
stringstyle=\ttfamily,

% Style for comments
commentstyle=\ttfamily,

moredelim=[is][\color{black}]{@@}{@},

literate=
    {α}{{\color{purple!35!black}\(\alpha\)\color{black}}}1
    {β}{{\color{purple!35!black}\(\beta\)\color{black}}}1
    {⪯}{\(\preceq\)}1
    {≤}{\(\le\)}1
    {→}{\(\to\)}2
    {∀}{\(\forall\)}1
    {∃}{\(\exists\)}1
    {'}{{\!'}}1
    {«}{{\guillemotleft}}1
    {»}{{\guillemotright}}1
}

